Quantum Generative Adversarial Networks For Anomaly Detection In High Energy Physics

The standard model (SM) of particle physics represents a theoretical paradigm for the description of the fundamental forces of nature. Despite its broad applicability, the SM does not enable the description of all physically possible events. The detection of events that cannot be described by the SM, which are typically referred to as anomalous, and the related potential discovery of exotic physical phenomena is a non-trivial task. The challenge becomes even greater with next-generation colliders that will produce even more events with additional levels of complexity. The additional data complexity motivates the search for unsupervised anomaly detection methods that do not require prior knowledge about the underlying models. In this work, we develop such a technique. More explicitly, we employ a quantum generative adversarial network to identify anomalous events. The method learns the background distribution from SM data and, then, determines whether a given event is characteristic for the learned background distribution. The proposed quantum-powered anomaly detection strategy is tested on proof-of-principle examples using numerical simulations and IBM Quantum processors. We find that the quantum generative techniques using ten times fewer training data samples can yield comparable accuracy to the classical counterpart for the detection of the Graviton and Higgs particles. Additionally, we empirically compute the capacity of the quantum model and observe an improved expressivity compared to its classical counterpart.

==> acronyms.tex <==
\newacronym{auc}{AUC}{Area Under Curve}
\newacronym{bsm}{BSM}{Beyond the Standard Model}

\newacronym{cm}{CM}{center of mass}
\newacronym{cern}{CERN}{European Organization for Nuclear Research}
%Conseil Européene pour la Recherche Nucléaire

\newacronym{dtc}{DTC}{Decision Tree Classifier}
\newacronym{gbc}{GBC}{Gradient Boosting Classifier}

\newacronym{hep}{HEP}{high energy physics}
\newacronym{hlf}{HLF}{high level feature}
\newacronym{hlt}{HLT}{high level trigger}
\newacronym{hl-lhc}{HL-LHC}{High Luminosity Large Hadron Collider}
\newacronym{lep}{LEP}{Large Electron-Positron Collider}
\newacronym{lhc}{LHC}{Large Hadron Collider}
\newacronym{cms}{CMS}{Compact Muon Solenoid}
\newacronym{mcc}{MCC}{Matthews Correlation Coefficient}
\newacronym{met}{MET}{missing transverse energy}
\newacronym{ml}{ML}{machine learning}

\newacronym{nisq}{NISQ}{Noisy Intermediate-Scale Quantum}

\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{pf}{PF}{particle-flow}

\newacronym{rfc}{RFC}{Random Forest Classifier}
\newacronym{roc}{ROC}{Receiver Operator Characteristics}

\newacronym{slac}{SLAC}{Stanford Linear Accelerator Center}
\newacronym{sm}{SM}{Standard Model}
\newacronym{susy}{SUSY}{Supersymmetry}

\newacronym{svm}{SVM}{Support Vector Machine}

\newacronym{qed}{QED}{Quantum Electrodynamics}
\newacronym{qft}{QFT}{Quantum Field Theory}
\newacronym{qml}{QML}{Quantum Machine Learning}
\newacronym{qsvm}{QSVM}{Quantum Support Vector Machine}

\newacronym{vbf}{VBF}{vector boson fusion}
\newacronym{vqc}{VQC}{Variational Quantum Classifier}

\newacronym{qgan}{qGAN}{Quantum Generative Adversarial Networks}
\newacronym{gan}{GAN}{Generative Adversarial Networks}
\newacronym{wgan}{WGAN}{Wasserstein Generative Adversarial Networks}

\newacronym{sgd}{SGD}{Stochastic Gradient Descent}
